Detections of interstellar 2-cyanopyrene and 4-cyanopyrene in TMC-1

Polycyclic aromatic hydrocarbons (PAHs) are among the most ubiquitous compounds in the universe, accounting for up to ~25% of all interstellar carbon. Since most unsubstituted PAHs do not possess permanent dipole moments, they are invisible to radio astronomy. Constraining their abundances relies on the detection of polar chemical proxies, such as aromatic nitriles. We report the detection of 2- and 4-cyanopyrene, isomers of the recently detected 1-cyanopyrene. We find that these isomers are present in an abundance ratio of ~2:1:2, which mirrors the number of equivalent sites available for CN addition. We conclude that there is evidence that the cyanopyrene isomers formed by direct CN addition to pyrene under kinetic control in hydrogen-rich gas at 10 K and discuss constraints on the H/CN ratio for PAHs in TMC-1.

==> calculations_TS_RW.tex <==
!!!!!The numbers in here will be adjusted to match the refined values!!!!


The use of cyano-pyrene abundance to estimate the abundance of pyrene relies on knowledge of the pathway to the formation of cyano-pyrene. If cyano-pyrene is formed directly from the reaction of CN radicals with pyrene then its relative abundance will be strongly related to the rate coefficient for CN with pyrene, as well as its destruction pathways. Where production of cyano-pyrenes are dominated by the CN addition to pyrene under kinetic control it is reasonable to expect the branching ratio to be related to the number of equivalent sites, due to the absence of any dipole moment. Calculations were therefore carried out to evaluate if the observed isomer distribution is in agreement with kinetic control from addition of CN to pyrene. 

Computational methods:

Initial structures for the adducts and separated reagents were optimized with the RI-BP86 DFT functional \cite{Parr_88} using the def2-SVP basis set \cite{Ahlrichs_2005} and including D3(BJ) empirical dispersion corrections \cite{Goerigk_2011}. The presence of barriers to subsequent transfer and elimination from the adducts were evaluated using relaxed surfaces scans with RI-BP86-D3(BJ)/def2-SVP; where peaks in the scans were observed these were used as the initial guess for transition state optimizations. No barriers were observed for the addition of CN to the ring in the 1, 2 or 4 position to verify this result, additional relaxed scans with the more reliable hybrid functionals and triple zeta basis sets $\omega$B97X-D4/def2-TZVPP \cite{Head-Gordon_2008, Weigend_2006, Grimme_2017} and M06-2X/def2-TZVPP \cite{Truhlar_2008, Weigend_2006} were carried out. All the structures calculated previously were then further refined and harmonic vibrations were calculated with the $\omega$B97X functional \cite{Head-Gordon_2008} with the triple zeta basis set def2-TZVPP \cite{Weigend_2006} and D4 empirical dispersion corrections \cite{Grimme_2017}. Single point energy corrections for these were then carried out using the EP3 approximation of the CCSD(T) complete basis set limit \cite{Hobza_2006,Neese_2012}. This approach can yield accuracy on the order of 5 -- 10 kJ mol$^{-1}$ with the accuracy of the relative energies of similar species (the 3 isomers formed for example) likely to be much higher on the order of \pm 1 kJ mol$^{-1}$. All these calculations were performed using ORCA 5.0.4 \cite{Neese_2022}. 
\begin{equation}
Equation 1: CCSD(T)/CBS \approx EP3 = E_HFCBS + E_MP2CBS + E_CCSD(T)small - E_MP2small 
\end{equation}

The results of this work show that the approach of CN to pyrene is barrierless for the addition of carbon to the 1, 2 or 4 positions, leading to the formation of deeply bound adducts 190 -- 250 kJ mol$^{-1}$ below the entrance energies. The barriers to the subsequent H atom elimination are submerged by 70 -- 80 kJ mol$^{-1}$.

Master equation 

This EP3//$\omega$B97X-D4/def2-TZVPP surface was then incorporated into the energy-grained master equation calculator MESMER 7.0 \cite{Robertson_2012} which allowed for the reaction to be simulated over a range of pressures and temperatures. There are 8 equivalent pathways to addition at the 1 and 4 positions and 4 equivalent pathways to addition at the 2 position leading to a  The temperature-dependent collision limit for CN and Pyrene was estimated using:
%\cite{West_2019}

\begin{equation}
    k_{\textrm{coll}(T)} = \sigma_{\textrm{coll}}\langle v(T) \rangle 
\end{equation}
this was then treated with the inverse Laplace transformation  (ILT) methodology \cite {Pilling_1986} in MESMER along with RRKM treatment \cite{Robertson_1996,Hase_1996,Hase_2009} for the H atom elimination reactions. The A factor for the ILT into the individual adduct wells was set to the fraction of the total number of pathways available that led to the formation of that isomer.

This model predicts that at 10 K and \leq 1 \times 10$^{10}$ cm$^{-3}$ the barriers to H elimination are sufficiently submerged for prompt H atom formation following CN addition to the ring. Therefore, this leads to the formation of 1-, 2- and 4-cyanopyrene in a  2:1:2 ratio. The site-specific bi-molecular removal rate coefficients at 10 K are predicted to be \textit{k$_1$} = 2.07 \times 10$^{-10}$ cm$^3$ s$^{-1}$, \textit{k$_2$} = 1.03 \times 10$^{-10}$ cm$^3$ s$^-1$, \textit{k$_4$} = 2.06 \times 10$^{-10}$ cm$^3$ s$^{-1}$.


\begin{table}
    \centering
    \begin{tabular}{cccccc}
         &  wB97XD4 &  sZPE&  DH 0K / kJ mol-1&  EP3& DH0K / kJ mol-1\\
         CN + Pyrene&  -709.04756859
&  0.20531153
&  0&  -707.51552912
& 0\\
         Adduct - 1 &  -709.14549706
&  0.20795853
&  -250.161
&  & \\
         Adduct - 2&  -709.12292909
&  0.20727361
&  -192.708
&  & \\
         Adduct - 4&  -709.14131632
&  0.20802809
&  -239.002
&  & \\
         TS e1&  -709.07873496
&  0.20081908
&  -93.622
&  & \\
         TS e2&  -709.07323909
&  0.20078966
&  -79.270
&  & \\
         TS e4&  -709.07796105
&  0.20087818
&  -91.435
&  & \\
         H + 1-Cyanopyrene&  -709.08858469
&  0.19944984
&  -123.078
&  -707.54954531
& -104.699
\\
         H+ 2-Cyanopyrene&  -709.08692346
&  0.19930482
&  -119.097
&  -707.54795048
& -100.893
\\
 H + 4 Cyanopyrene& -709.08783089
& 0.19942930
& -121.152
& -707.54887256
&-102.987
\\
    \end{tabular}
    \caption{Energetics of the CN + Pyrene reaction at the  EP3//$\omega$B97X-D4/def2-TZVPP level  }
    \label{tab:my_label}
\end{table}


Ignore this second table unless you think there is some value in it, would need additional lines to explain  the methods

\begin{table}
    \centering
    \begin{tabular}{ccccl}
 & wB97X-D4/def2-TZVPP& EP3//&DLPNO-CCSD(T)/CBS// &CCSD(T)-F12b/cc-pVDZ-F12//\\
         1-Cyanopyrene&  0.00&  0.00&  0.00&0.00\\
         2-Cyanopyrene&  3.98&  3.81&  2.95&3.46\\
         4-Cyanopyrene&  1.93&  1.71&  0.59&1.72\\
    \end{tabular}
    \caption{Relative enthalpies of  formation of the isomers at 0K in kJ mol$^{-1}$ }
    \label{tab:RelIsomerE}
\end{table}


\begin{table}
    \centering
    \begin{tabular}{ccccccc}
 & \multicolumn{2}{c}{1-cyanopyrene}& \multicolumn{2}{c}{2-cyanopyrene}& \multicolumn{2}{c}{4-cyanopyrene}\\
         &  $\beta$&  $\gamma$&  $\beta$&  $\gamma$&  $\beta$& $\gamma$\\
         H+
&  1.30E-08&  3.33E+00&  1.30E-08&  3.53E+00&  1.29E-08& 3.16E+00
\\
         H3+
&  7.54E-09&  3.33E+00&  7.55E-09&  3.53E+00&  7.49E-09& 3.16E+00
\\
         He+
&  6.54E-09&  3.33E+00&  6.55E-09&  3.53E+00&  6.50E-09& 3.16E+00
\\
         C+
&  3.84E-09&  3.33E+00&  3.85E-09&  3.53E+00&  3.81E-09& 3.16E+00
\\
 HCO+
& 2.55E-09& 3.33E+00& 2.56E-09& 3.53E+00& 2.53E-09&3.16E+00
\\
    \end{tabular}
    \caption{kSC parameters for selected ion molecule reactions with the 1, 2, and 4-cyanopyrene isomers  }
    \label{tab:CyanoPyreneRemovalRates}
\end{table}
